AI-Driven Confidential Computing across Edge-to-Cloud Continuum

With the meteoric growth of technology, individuals and organizations are widely adopting cloud services to mitigate the burdens of maintenance. Despite its scalability and ease of use, many users who own sensitive data refrain from fully utilizing cloud services due to confidentiality concerns. Maintaining data confidentiality for data at rest and in transit has been widely explored but data remains vulnerable in the cloud while it is in use. This vulnerability is further elevated once the scope of computing spans across the edge-to-cloud continuum. Accordingly, the goal of this dissertation is to enable data confidentiality by adopting confidential computing across the continuum. Towards this goal, one approach we explore is to separate the intelligence aspect of data processing from the pattern-matching aspect. We present our approach to make confidential data clustering on the cloud, and then develop confidential search service across edge-to-cloud for unstructured text data. Our proposed clustering solution named ClusPr, performs topic-based clustering for static and dynamic datasets that improves cluster coherency up to 30%-to-60% when compared with other encryption-based clustering techniques. Our trusted enterprise search service named SAED, provides context-aware and personalized semantic search over confidential data across the continuum. We realized that enabling confidential computing across edge-to-cloud requires major contribution from the edge tiers particularly to run multiple Deep Learning (DL) services concurrently. This raises memory contention on the edge tier. To resolve this, we develop Edge-MultiAI framework to manage Neural Network (NN) models of DL applications such that it can meet the latency constraints of the DL applications without compromising inference accuracy.

==> B-abstract.tex <==
With the  meteoric growth of technology, 
both individuals and organizations are widely adopting cloud services to mitigate the burdens of maintenance. Despite its scalability and ease of use, many potential cloud users who own sensitive data refrain from fully utilizing cloud services due to valid confidentiality concerns. Maintaining data confidentiality for data at rest and in transit has been widely explored but data remains vulnerable in the cloud while it is in use. This vulnerability is further elevated once the scope of computing spans across the edge-to-cloud continuum.  From the notion of safeguarding, confidential data needs to be encrypted while offloading from users' premises. Although adopting user-side encryption ensures data confidentiality, it limits the ability to data processing. Subsequently, we are limited to performing only low-level operations (\eg string pattern matching). Accordingly, the goal of this dissertation is to enable data confidentiality by adopting confidential computing across the continuum. Towards this goal, one approach we explore is to separate the intelligence aspect of data processing from the pattern-matching aspect. We present our approach to make confidential data clustering on the cloud, and then develop  confidential search service across edge-to-cloud for unstructured text data. Our proposed clustering solution named ClusPr, performs topic-based clustering for static and  dynamic datasets that improves cluster coherency up to 30\%-to-60\% when compared with other encryption-based clustering techniques. Our trusted enterprise search service named SAED, provides context-aware and personalized semantic search over confidential data across the continuum. Evaluation results, verified by human users, demonstrates that SAED can improve
the relevancy of the retrieved search results by $\approx$ 24\% for plain-text and 75\% for encrypted  datasets. We realized that enabling confidential computing across edge-to-cloud requires major contribution from the edge tiers particularly to run multiple Deep Learning (DL) services concurrently. This raises memory contention on the edge tier. To resolve the contention, we propose Edge-MultiAI framework to manage Neural Network (NN) models of DL applications such that it can meet the latency constraints of the DL applications without compromising inference accuracy. Our evaluation confirms that Edge-MultiAI can stimulate the degree of multi-tenancy by $2\times$ on the edge tier.


==> B-acknowledgement.tex <==
~
            I sincerely thank my supervisor, Dr. \Supervisor, for his constant encouragement since the inception of the journey. He has provided a plethora of guidance, support, and cooperation. Thanks to my dissertation committee, Dr. Raju Gottumukukkala, Dr. Li Chen, Dr. Xiali Hei, and Dr. Sheng Chen. Thanks to Jason Woodworth, Razin Farhan Hussain, Davood Ghatreh Samani, and Chavit Denninart for their assistance in the work of this dissertation. A special thanks goes to Ali Mokhtari for his collaboration in the latest work. Finally, thanks goes to the Center for Advanced Computer Studies and the Graduate School at the University of Louisiana at Lafayette for their support and guidance.


==> B-dedicatory.tex <==
\vspace*{\fill}
\begin{center}
\textit{
To my Creator, the Almighty Allah (SWT), my master prophet Muhammad (pbuh), who taught us the purpose of life, my parents, Md Mazharul Islam and Jubaida Naznin, who never stop providing support in countless ways, my enlighteners, Md Fazle Rabby, Md Sazib Hasan who have provided enormous inspiration regardless of the rainy or shiny days throughout the journey with the fullest and truest attention, my pioneer since childhood, Jahid Md Mahabub Islam, who has been acting as a LiDAR through the sea of darkness, my asymptotic remembrance, Farzana Hasan, whom I am forever grateful, my mentors, Muhammad Usama Islam, Md Istiaq Hossain, Jubair Yusuf, Farhan Tanvir, my only sister, Mantika Mahbuba, and to all my friends and beloved ones.   
}
\end{center}
\vspace*{\fill}



==> C1-Intro.tex <==
\chapter{Introduction}


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/C1/smartOilField.pdf}
%     \caption{A remote offshore smart oil field consist of multiple oil rigs(oil extraction sites). Each of the oil rigs have edge computing system to support it's own computing demands (\eg report generation, oil spill detection, toxic gas detection)}
%     \label{fig:C1intro2}
% \end{figure}


The expeditious growth of digitalization has been producing a massive volume of data, known as \emph{big data}, in both structured and unstructured formats. In every seconds, more than 1.7 megabytes of new data is
created for every human in form of the outputs of IoT-based
sensors, organizational documentation, RSS feed, transaction
record, digital content, social media activities,
and so on. %The volume of data is growing faster than ever before and subsequently, it is expected that world’s total data volume will exceed 149 zetabytes by the next three years.
It is estimated that every day 2.5 Exabytes of data are being generated in which, over 80\% of the data is in unstructured (\eg audio, streaming, text) form~\cite{clustcrypt}.
Cloud services have been effective in relieving big data owners from the burden of maintaining and accessing these data.
%Likewise, cloud providers began offering \emph{enterprise search} services that enable data owners to semantically search over their datasets in the cloud (\eg AWS Kendra~\cite{kendra}).
However, in spite of the advantages of the cloud services, many potential data owners especially, dealing with privacy-preserving data, are hesitant to shift to cloud due to valid data-privacy concerns~\cite{S3BD,al2019cybersecurity} on the cloud servers, particularly after numerous recent privacy violations~\cite{cloudacci,zobaedbig}. 
Therefore, data integrity in the cloud is another security concern. The challenge is how to verify the data integrity in the cloud storage without downloading and then uploading the data back to cloud. Rapid incoming of new data to the cloud, makes verifying data integrity further complicated (\cite{chen2012data}). Techniques such as continuous integrity monitoring are applied to deal with big data integrity challenge in the cloud (\cite{lebdaoui2016managing}) nonetheless they are not effective.

 % Please add the following required packages to your document preamble:
% \usepackage{multirow}

An ideal privacy-preserving solution for such clients (\ie data owner) will enable them to securely utilize cloud services, while providing access ability only to authorized users, potentially from thin-clients (\eg %hand-held devices and 
smartphones) with storage, energy, and data processing constraints.

%MODIFY FROM HERE

Client-side encryption~\cite{kaaniche2014secure}, %litwin2011privacy}, 
in which documents are encrypted with private keys before outsourcing them to the cloud, is a promising approach to achieve data privacy.
In this method, only the client has the ability to decrypt the documents, hence, it can potentially provide confidentiality against both internal and external attackers~\cite{kaaniche2014secure,zobaedbig}. However, the limitation of this method is the lack of processing (\eg clustering and search) ability on the encrypted documents while maintaining latency sensitivity. In addition, adopting only an encryption technique while data is at rest in storage or transmit does not ensure data privacy violation when the data is accessed (in memory). Subsequently, the ability to protect data and executables (code) while they are in use is limited in conventional computing environment.
In this regard, the idea of confidential computing comes forward that enables the creation of a hardware enforced trusted execution environment (TEE) for secure computing (\eg data analytics) without tempering data privacy. These isolated environments prevent unauthorized access or modification of executables and data while in use. By that means, confidential computing enhances the security assurances for organizations that deal with privacy-preserving data.  



Recently, cloud providers has begun offering different enterprise services that enable data  owners to access (\eg analytics, inferencing) their datasets in the cloud. For instance, AWS has launched an enterprise search service named Kendra~\cite{kendra} that offers real-time semantic searchability using state-of-the-art natural language modeling techniques. However, such services can work only over plain-text dataset~\cite{zobaed2021saed}. It is noteworthy to mention that throughout this research, we consider only the text-based unstructured data.


In the context of trustworthy text-based data processing, searchable encryption systems (\eg~\cite{pham2019survey, zhang2020lightweight,zhang2020se,salehi2017reseed}) have been developed to enable privacy preserving search ability over the encrypted data. Such systems predominantly extract keywords (aka tokens) from documents to build an encrypted index, which is  traversed against a search query at the search time to find relevant documents. The problem arises for big datasets where the index structure is prohibitively large, such that traversing it becomes the search bottleneck~\cite{S3BD}. As an instance, for a 100 petabytes dataset, in S3C~\cite{S3C} search tool, %which is a secure semantic search tool, 
the size of index grows to $\approx$ 300 GB. Traversing such a large index affects searching timeliness %of the search 
and can potentially be impacted by hardware capabilities~\cite{salehi2017reseed}. To resolve the bottleneck, the index structure commonly is partitioned to several \emph{clusters}~\cite{XuCroft, Google}. Later, based on a given search query, search space is pruned to search on the clusters that are relevant to the query for faster operation. 

Moreover, the dataset could have static or dynamic characteristics.~\textit{Static dataset} as the one that remains unchanged, once it is uploaded to the cloud such as obsoleted data (\eg HUB5~\cite{da}), archived data (\eg ACCC, RFC~\cite{S3BD}), newsgroup data, book contents, and so on. Alternatively, a \textit{dynamic dataset} refers to the ones whose document set grows or shrinks over time, such as criminal records~\cite{sa2}, digital libraries~\cite{moma21}, and social network feeds~\cite{sa3}. 

Encrypted data processing or analytics methods are challenging because the data semantic is lost, once it is encrypted.  Clustering is one of the crucial data analytics methods that are commonly used to group datapoints based on their shared attributes. The clustering challenge gets further complicated if we need to cluster encrypted data containing dynamism property. 
These difficulties often make the data accessibility ill-suited for big-data-scale datasets. 

To reduce the computing burden of thin-clients, on-premise \emph{Edge computing}~\cite{sahan2019edge,nur2019priority,zobaed2021saed} can be leveraged for facilitating data processing: cleaning, formatting, missing values, data analytics: clustering, semantic expansion, inferencing, visualization, and data encryption to pace with real-timeliness constraint. Figure~\ref{fig:C1intro1} represents workflow from big data generation at user end and pre-processing them on the edge node to perform analytics on the cloud.
However, maintaining trustworthiness across edge to cloud to facilitate confidential computing imposes a new challenge. 
This thesis offers a solution to address these problems.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{figures/C1/client_edge_cloud2.pdf}
    \caption{High-level workflow diagram of big data generation and pre-processing them on the edge to big data storage and analytics on the cloud.}
    \label{fig:C1intro1}
\end{figure}
\section{Motivation: Confidential Computing of Unstructured Data}
The motivation for this research is an organization with a massive volume of privacy-preserving unstructured data that are often in the form of text.   Such organization would have users who need searching semantically over the data in real-time.
% Add lines related to confidential computing 
One instance of such organization is a law enforcement agency with encrypted
crime report data, with officers who would require to search over the reports using their handheld devices while at the office or on the move in real-time. Searching exhaustively over the whole index for a given search query prohibits the real-timeliness search constraint. Therefore, index partitioning (aka clustering) is required to prune the search space so that search can be performed over a pruned index with minimal overhead. 

The officers may not remember exact keywords in the documents they are searching for. Hence, they need to retrieve documents semantically and contextually related to their given search query.
As example, if a officer searches for ``robbery'', he  can also be interested in finding documents about ``mugging'', ``theft'', or ``break in". Moreover, the officer can desire for personalized search. 

In addition, since the officer performs the searches on their limited resourceful handheld devices in real-time, the solution should incur a minimal processing overhead and scale well to massive amount of text data.


To this end, a robust and secure enterprise search service is the need of the hour to search semantically over the encrypted privacy-preserving data in real-time. In Figure~\ref{fig:C1intro1.1}, a high-level architecture of secure enterprise search service is depicted. Such service provides the secure search intelligence utilizing the on-premises edge resources. The high-end storage and compute resources on the cloud tier are utilized by the existing enterprise search systems to exhaustively carry out pattern matching on the entire dataset.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/C1/client_edge_cloud.pdf}
    \caption{A high-level diagram of user-edge-cloud based three-tier architecture to facilitate smart and privacy-preserving enterprise search service.}
    \label{fig:C1intro1.1}
\end{figure}
 
 %added
 \section{Motivation: Edge Multi-Tenancy for Latency Sensitive Processing }
 An edge server is an indispensable part of an IoT-based system that has to continuously execute multiple (a.k.a. multi-tenant) smart (\eg deep learning) applications with low-latency and
high accuracy. However, due to memory limitation, executing latency-sensitive multi-tenant applications on an edge server can cause memory contention problem that decreases execution rate. This is because, DL applications utilize bulky Neural Network (NN) models at their kernel to infer on the inputs received from the sensors. The NN models have to be kept in memory to enable low-latency (a.k.a. \emph{warm-start}~\cite{dang2017dtrust}) inference operations. Otherwise, because the NN model size is often huge, loading it into the memory in an on-demand manner (a.k.a. \emph{cold-start}) is counterproductive and affects the latency constraint of the DL applications. As the edge servers naturally have a limited memory size (\eg 4 GB in the case of Jetson Nano \cite{nvidia}), multi-tenant execution of DL applications on them leads to a memory contention challenge across the processes~\cite{deng2020edge,gholami2021survey}.
%This is because, DL applications function based on bulky neural network (NN) models that cannot be simultaneously maintained in the limited memory space of the edge. 

To this point, in a multi-tenant execution environment, it is crucial to load a model in memory while executing a particular application such that loading the new model does not hamper other ongoing (\ie active) multi-tenant executions.  
 
\section{Research Problem and Objectives}
With the aim of facilitating trustworthy natural language processing across edge to cloud continuum, in this dissertation, we address the following research problems:

\begin{enumerate}
\item How to optimally and scalably cluster keywords in an encrypted big dataset? In other words, how to topically prune the searchable encryption index?  
\item How to manage the clusters if the data contains dynamism? 
\item  How to search semantically over encrypted data with minimum overhead?
\item How to develop a trustful robust encrypted enterprise search service?
\item How to manage models of trustworthy DL applications to stimulate multi-tenancy without compromising their inference accuracy?

\end{enumerate}

\section{Contributions} 
Considering the research questions described in the previous section, the
major \textbf{contributions} of this dissertation are:
\begin{enumerate}
 \item We propose a method to estimate the suitable number of clusters (\textit{K}) needed to partition a given encrypted dataset. %(see \cref{subsec:kestimate} ).
    \item To enable privacy-preserving clustering in the cloud, we develop three clustering schemes (namely, S-ClusPr, SD-ClusPr, and FD-ClusPr) that can cluster encrypted data across static, semi-dynamic, and fully-dynamic unstructured datasets, respectively.% (see \cref{subsec:sdcs}, \cref{subsec:fdcs}).
    \item We evaluate and analyze the developed clustering schemes against both encrypted and plain-text clustering approaches with respect to the cluster goodness metrics. % (see \cref{subsec:evaluationres}).
    
    \item We develop an open-source mechanism (titled as \emph{SAED}) at the edge tier that offers personalized semantic searchability on existing cloud-based enterprise search services in real-time while maintaining data privacy.
    \item We design a method for proactive query expansion to cover the search semantic with respect to its context. In addition, we develop a method based on a recurrent neural network model to personalize the search via assigning a weight to each expanded query. 
    
    \item We evaluate the search accuracy and privacy of SAED via
plugging it to the existing cloud-based search services.

   \item We develop an NN model management framework for multi-tenant DL applications on the edge server, called \emph{Edge-MultiAI}, that efficiently utilizes the memory such that the multi-tenancy degree and number of warm-start inferences are maximized without any major compromise on the inference accuracy. Edge-MultiAI dynamically loads the high-precision NN model for the requester application, while loading low-precision ones for others.
 
    \item  We develop \emph{iWS-BF}E policy along with three other baseline heuristic policies within Edge-MultiAI to choose the suitable model for the application performing inference, and to decide how to allocate memory for it. 
    
    \item We evaluate and analyze the efficacy of the proposed heuristics in terms of their effectiveness and robustness against uncertainties in the inference request prediction.

\end{enumerate}
\section{Dissertation Organization }
%HERE
\begin{itemize}
\item Chapter~\ref{chap:bg} provides background for: big data \& confidential computing in the cloud, trustworthy natural language processing (NLP), smart query processing, and scope of edge computing for trustworthy NLP and explores the related research works.

\begin{itemize}
     \item \textbf{Sm Zobaed}, Mohsen Amini Salehi,
     \textit{Big Data in the Cloud} published in Encyclopedia of Big data, Springer, ISBN: 978-3-319-32009-0.
     \item \textbf{Sm Zobaed}, Md Enamul Haque, Md Fazle Rabby, Mohsen Amini Salehi,
     \textit{Senspick: Sense Picking for Word Sense Disambiguation}, Published in proceedings of the 15th IEEE International Conference on Semantic Computing (ICSC'21), Online, 2021.
          \item \textbf{Sm Zobaed}, Mohsen Amini Salehi,
     \textit{A Survey on Confidential Computing over Edge to Cloud Continuum}, Preparing to be submitted.
\end{itemize}

\item Chapter~\ref{chap:clus} explores the Benefits of clustering privacy-preserving text-based big data. The semantics of the data is lost after the encryption. However, the data can be clustered topically %without the necessity of semantic knowledge,  
by utilizing the statistical characteristics of the data. This Chapter discusses our proposed approach of clustering encrypted static and dynamic data. In addition, the Chapter compares the clusters obtained by proposed approach and others in the measure of popular cluster goodness metrics (\eg Silhouette Coefficient, Davis-Boudin index). Finally, it presents a set of experiments carried out in a realistic environment to show the effectiveness of the clustering. 
\begin{itemize}
\item \textbf{Sm Zobaed}, Sahan Ahmad, Raju Gottumukkala, Mohsen Amini Salehi,
\textit{Clustcrypt: Privacy-preserving clustering of unstructured big data in the cloud}, Published in proceedings of the 21st IEEE International Conference on High Performance Computing and Communications (HPCC'19), China, 2019.  (Full code in Github repository: https://github.com/hpcclab/ClustCrypt).
\item Sahan Ahmad, \textbf{Sm Zobaed}, Raju Gottumukkala, Mohsen Amini Salehi,
\textit{Edge Computing for User-Centric Secure Search on Cloud-Based Encrypted Big Data}, Published in proceedings of the 21st IEEE International Conference on High Performance Computing and Communications (HPCC'19), China, 2019.
\item \textbf{Sm Zobaed}, Mohsen Amini Salehi,
\textit{Privacy-Preserving Clustering of Unstructured Big Data for Cloud-Based Enterprise Search Solutions}, Submitted (In revision stage) in Journal of Concurrency and Computation: Practice and Experience (CCPE), 2022. (Full code in Github repository: https://github.com/zobaed11/Jorunal-Version).
\end{itemize}

\item  Chapter~\ref{chap:saed} studies the significance of secure and personalized semantic search over the encrypted data. This Chapter explains the workflow and mechanisms of the proposed secure search service architecture. Finally, it presents a set of experiments carried out in AWS Kendra service environment to show the effectiveness of the search relevancy.
\begin{itemize}
\item \textbf{Sm Zobaed}, Mohsen Amini Salehi, Rajkumar Buyya,
\textit{SAED: Edge-Based Intelligence for Privacy-Preserving Enterprise Search on the Cloud}, Published in proceedings of the 21st ACM/IEEE International Conference on Cluster Cloud and Grid Computing (CCGrid ’21), Australia, 2021. 
(Full code in Github repository: https://github.com/hpcclab/SAED-Security-At-Edge)
\end{itemize}
\item Chapter~\ref{chap:concurrent} explores multi-tenant execution of latency-sensitive DL applications on resource constraint edge devices.

\item Chapter~\ref{chap:conc} concludes the dissertation with a discussion of our main findings.

\item Chapter~\ref{chap:future} explores further research topics and directions that emerged during the course of this research but have not discussed in this thesis.

\end{itemize}

==> F-abstract.tex <==
\setlinespacing{1}
 \begin{description}
    \setlength{\parsep}{-3pt}
    \setlength{\itemsep}{-1.7pt}
    \setlength{\parindent}{0pt}
    \setlength{\labelsep}{-5pt}
    \item Zobaed, Sm.$\ $ 
                Bachelor of Science in Computer Science and Engineering, Islamic University of Technology, 2015;
                Master of Science, University of Louisiana at Lafayette,
                2019;
                Doctor of Philosophy, University of Louisiana at Lafayette,
                2022
    \item Major:$\ $                  \Major
    \item Title of Dissertation:$\ $  \Title
    \item Dissertation Director:$\ $  \Supervisor
    \item Pages in Dissertation:$\ $  180;  Words in Abstract:$\ $  347 %% UL limit it to 350
 \end{description}
\setlinespacing{1}
 \begin{theabstract}
 	\indent
                With the  meteoric growth of technology, 
both individuals to organizations are widely adopting cloud services to mitigate the burdens of maintenance. Despite its scalability and ease of use, many potential cloud users who own sensitive data refrain from fully utilizing cloud services due to valid confidentiality concerns. Maintaining data confidentiality for data at rest and in transit has been widely explored but data remains vulnerable in the cloud while it is in use. This vulnerability is further elevated once the scope of computing spans across the edge-to-cloud continuum.  From the notion of safeguarding, confidential data needs to be encrypted while offloading from users' premises. Although adopting user-side encryption ensures data confidentiality, it limits the ability to data processing. Subsequently, we are limited to performing only low-level operations (\eg string pattern matching). Accordingly, the goal of this dissertation is to enable data confidentiality by adopting confidential computing across the continuum. Towards this goal, one approach we explore is to separate the intelligence aspect of data processing from the pattern-matching aspect. We present our approach to make confidential data clustering on the cloud, and then develop  confidential search service across edge-to-cloud for unstructured text data. Our proposed clustering solution named ClusPr, performs topic-based clustering for static and  dynamic datasets that imposes cluster coherency upto 30\%-to-60\% when compared with other encyption-based clustering techniques. Our trusted enterprise search service named SAED, provides context-aware and personalized semantic search over confidential data across the continuum. Evaluation results, verified by human users, demonstrates that SAED can improve
the relevancy of the retrieved search results by $\approx$ 24\% for plain-text and 75\% for encrypted  datasets. We realized that enabling confidential computing across edge-to-cloud requires major contribution from the edge tiers particularly to run multiple Deep Learning (DL) services concurrently. This raises memory contention on the edge tier. To resolve the contention, we propose Edge-MultiAI framework to manage NN models of DL applications such that it can meet the latency constraints of the DL applications without compromising inference accuracy. Our evaluation confirms that Edge-MultiAI can stimulate the degree of multi-tenancy by $2\times$ on the edge tier.


\end{theabstract}

